Embedded vs. External Controllers in Software-Defined IoT Networks

The flexible and programmable architectural model offered by Software-Defined Networking (SDN) has re-imagined modern networks. Supported by powerful hardware and high-speed communications between devices and the controller, SDN provides a means to virtualize control functionality and enable rapid network reconfiguration in response to dynamic application requirements. However, recent efforts to apply SDN's centralized control model to the Internet of Things (IoT) have identified significant challenges due to the constraints faced by embedded low-power devices and networks that reside at the IoT edge. In particular, reliance on external SDN controllers on the backbone network introduces a performance bottleneck (e.g., latency). To this end, we advocate a case for supporting Software-Defined IoT networks through the introduction of lightweight SDN controllers directly on the embedded hardware. We firstly explore the performance of two popular SDN implementations for IoT mesh networks, $\mu$SDN and SDN-WISE, showing the former demonstrates considerable gains over the latter. We consequently employ $\mu$SDN to conduct a study of embedded vs. external SDN controller performance. We highlight how the advantage of an embedded controller is reduced as the network scales, and quantify a point at which an external controller should be used for larger networks.

==> 5_RelatedWorks.tex <==
\subsection{Related Works} \label{sec:related_works}
In the previous section we discussed about design and working of two prominent architectures i.e. \usdn~~\cite{baddeley2018evolving} and \wise~\cite{\wise}. Apart from these architecture, there are a few other notable works. We will discuss about them briefly and also discuss about some of their shortcomings.

The authors of \wise facilitate~\cite{\wise-Onos} the heterogeneity characteristic of IoT by leveraging the Network Operating System (NOS). In their work an innovative integrated network operating system for the IoT which is obtained as the evolution of the Open Network Operating System (ONOS) is proposed. This integrated NOS allows the sensor nodes to interact with Openflow switches and vice-versa. The prototype is built using \wise architecture. This prototype helps in satisfying IoT characteristic of heterogeneity.

Some other works include CORAL-SDN~\cite{theodorou2017coralsdn}, which introduces centralized network mechanism to adjust protocol functionalities. It also proposes to introduce better network management and reduce resource utilization. They implement this by adapting SDN for IPv6 based \ieee RPL networks, and try  to deal with network overhead by reducing multiple RPL transmissions at beginning and thus provide more resources to SDN protocols.

Most of these architectures do not show any concrete comparisons in terms of it's performance with other existing SDN-IoT architecture. \usdn~\cite{baddeley2018evolving} shows some sort of comparison of performance with base RPL without SDN. Secondly, very few architectures have actual software implementation in Contiki OS many have implemented their work on hardware test beds. Finally, almost all architectures have customized controller suited for their architecture. \wise~\cite{\wise-Onos} integrated their architecture with ONOS a standard SDN controller but it was a technological demonstration and no extensive performance evaluation was carried out. We compare performance of two prominent architectures i.e. \usdn~\cite{baddeley2018evolving} and \wise~\cite{\wise}. After that we compare performance of \embedded controller and ONOS controller and provide appropriate reason for their performances. 
